Automated clustering of video games into groups with distinctive names

When doing a study on a large number of video games, it may be difficult to cluster them into coherent groups to better study them. In this paper, we introduce a novel algorithm, that takes as input any set of games S that are released on Steam and an integer k, and cluster S into k groups. Each group is then assigned a distinctive name in the form of a Steam tag. We believe our tool to be valuable for gaining deeper insights into the video game market. We show that our algorithm maximises an objective function that we introduce, the naming score, which assesses the quality of a clustering and how distinctive its name is.

==> tables/cluster_all.tex <==
\begin{table}[]
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
cluster name        & 2D                            & Open World            & Atmospheric                              & Multiplayer                      & Anime                      & Simulation                  & RPG                         & Sports            \\ \hline
naming score        & 1.14                          & 1.98                  & 1.11                                     & 1.01                             & 2.36                       & 1.67                        & 1.4                         & 2.7               \\ \hline
most reviewed games & Terraria                      & Grand Theft Auto V    & Dead by Daylight                         & Counter-Strike: Global Offensive & Wallpaper Engine           & Euro Truck Simulator 2      & The Witcher 3: Wild Hunt    & Rocket League     \\
                    & Stardew Valley                & Rust                  & Portal 2                                 & PUBG: BATTLEGROUNDS              & NARAKA: BLADEPOINT         & War Thunder                 & Warframe                    & EA SPORTS FIFA 23 \\
                    & Hollow Knight                 & ELDEN RING            & Sekiro: Shadows Die Twice - GOTY Edition & Dota 2                           & VRChat                     & Sid Meier's Civilization VI & Dying Light                 & FIFA 22           \\
                    & Geometry Dash                 & Cyberpunk 2077        & Deep Rock Galactic                       & Tom Clancy's Rainbow Six Siege   & Doki Doki Literature Club! & Cities: Skylines            & Baldur's Gate 3             & Assetto Corsa     \\
                    & The Binding of Isaac: Rebirth & ARK: Survival Evolved & Tomb Raider                              & Garry's Mod                      & Mirror 2: Project X        & RimWorld                    & The Elder Scrolls V: Skyrim & TEKKEN 7          \\ \hline
\end{tabular}
\caption{Clustering into $8$ clusters of the $4065$ games with at least $2000$ reviews, with their naming scores and the five most reviewed games for each cluster.}
\label{table:cluster_all}
\end{table}
